How Costly Was That (In)Decision?

In this paper, we introduce a new metric, named Penalty upon Decision (PuD), for measuring the impact of communication delays and state changes at the source on a remote decision maker. Specifically, the metric quantifies the performance degradation at the decision maker's side due to delayed, erroneous, and (possibly) missed decisions. We clarify the rationale for the metric and derive closed-form expressions for its average in M/GI/1 and M/GI/1/1 with blocking settings. Numerical results are then presented to support our expressions and to compare the infinite and zero buffer regimes. Interestingly, comparing these two settings sheds light on a buffer length design challenge that is essential to minimize the average PuD.

==> chapters/5-MM1K.tex <==
\section{M/M/1/K queue Analysis}\label{sec:MG11}
In this section, we show the theoretical analysis for M/M/1/K scheme where $K-1$ buffers exist for the queue and a packet will be dropped if it finds the buffers full. Therefore, we will have the missed decision probability equals to the probability that a packet arrives finding buffers full. In view of the renewal structure, we have the stationary distribution for M/M/1/K queue as:
\begin{align}
    p(i)=\frac{\rho^i}{\sum_{j=0}^{K}\rho^j}=\frac{\rho^i(1-\rho)}{1-\rho^{K+1}}.
\end{align}
where $p(i)$ is the probability that a packet arrives finding the queue with $i$ packets in it and $\rho=\frac{\lambda}{\mu}$ is the offered load of the system. Therefore, we have the missed probability as $p^M=p(K)=\frac{\rho^K(1-\rho)}{1-\rho^{K+1}}$
\begin{Theorem}
In M/M/1/K queue scheme, we have the correct and incorrect probability for the decisions made in the system as:
\begin{align}
	p^C&=,\\
	p^I&=.
\end{align}
\end{Theorem}
	\begin{Proof} The mathematical details can be found in Appendix.\ref{MM1K-P}.
\end{Proof}

We can also derive the correct and incorrect probability for all the generated packets as $p^C(1-p^M)$ and $p^I(1-p^M)$ respectively.

\begin{Theorem}
In M/M/1/K, we have the average correct and incorrect penalty for the decisions made in the system as:
\begin{align}
	\mathbb{E}[\sigma^C]&=,\\
	\mathbb{E}[\sigma^I]&=.
\end{align}
\end{Theorem}
	\begin{Proof} The mathematical details can be found in Appendix.\ref{MM1K-PA}.
\end{Proof}



